Diffusion Model for Data-Driven Black-Box Optimization

Generative AI has redefined artificial intelligence, enabling the creation of innovative content and customized solutions that drive business practices into a new era of efficiency and creativity. In this paper, we focus on diffusion models, a powerful generative AI technology, and investigate their potential for black-box optimization over complex structured variables. Consider the practical scenario where one wants to optimize some structured design in a high-dimensional space, based on massive unlabeled data (representing design variables) and a small labeled dataset. We study two practical types of labels: 1) noisy measurements of a real-valued reward function and 2) human preference based on pairwise comparisons. The goal is to generate new designs that are near-optimal and preserve the designed latent structures. Our proposed method reformulates the design optimization problem into a conditional sampling problem, which allows us to leverage the power of diffusion models for modeling complex distributions. In particular, we propose a reward-directed conditional diffusion model, to be trained on the mixed data, for sampling a near-optimal solution conditioned on high predicted rewards. Theoretically, we establish sub-optimality error bounds for the generated designs. The sub-optimality gap nearly matches the optimal guarantee in off-policy bandits, demonstrating the efficiency of reward-directed diffusion models for black-box optimization. Moreover, when the data admits a low-dimensional latent subspace structure, our model efficiently generates high-fidelity designs that closely respect the latent structure. We provide empirical experiments validating our model in decision-making and content-creation tasks.

==> sections/human_feedback.tex <==
\section{Off-policy bandit regret under human feedback}
We aim to learn the reward from human feedback and provide an upper bound for the off-policy bandit regret caused by the error inherited from reward estimation. Specifically, we assume a given dataset with human preference $\cD = \{(a_i, b_i, h_i)\}_{i\in[n]}$, here $a_i$ and $b_i$ are i.i.d. sampled from an unknown exploring policy $P_x$, and $h_i\in \{a_i, b_i\}$ is the human preference for $i\in[n]$. For simplicity, we also assume a linear reward, i.e. $r(x) = x^\top \theta^*$ for some $\theta = A\beta$, $\beta \in \mathbb{R}^d$ and $\|\beta\|_2 \leq 1$. We also assume low intrinsic dimension for the data sampling distribution: $a_i, b_i \in \cR(A)$. Following the Plackett-Luce model (PL model) \citep{cheng2010label,guiver2009bayesian,maystre2015fast}, we have the human preference probability given by $$
\P(h = a\mid a,b) = \frac{\exp(f^*(a))}{\exp(f^*(a)) + \exp(f^*(b))}.
$$
We use the following MLE to learn the underlying parameter $\hat{\theta}$: \begin{align*}
    \hat{\theta} =  \operatorname{argmin}_{\|\theta\|_2 \leq 1} l(\theta),
\end{align*}
where $$
l(\theta) := -\frac{1}{n} \sum_{i=1}^n \bigg\{ h_i^\top \theta - \log\bigg(\exp(a_i^\top \theta ) + \exp(b_i^\top \theta)\bigg) \bigg\}.
$$
We also define the off-policy bandit regret as $\EE_{x\sim P_a}[|\hat{f}(x) - f^*(x)|]$, which is a crucial term in the suboptimality of reward diffusion. We now present our results.
\begin{theorem}\label{thm:rew-hf-est}
    With probability at least $1-\delta$, we have \begin{align*}
        \EE_{x\sim P_a}[|\hat{f}(x) - f^*(x)|] \leq O\bigg(\sqrt{\kappa^2\cdot \frac{d+\log1/\delta}{n}+ \lambda} \cdot \sqrt{ \operatorname{Tr}(\EE_{P_a}[z z^\top] (\Sigma_z + \lambda I_d)^{-1} )}\bigg)
    \end{align*}
    here $\kappa = \big(1+\exp(\sqrt{\log n / \delta})\big)^2$, and $\Sigma_z  = \frac{1}{n} \sum_{i=1}^n A^\top(a_i - b_i)(a_i - b_i)^\top A^\top$.
\end{theorem}
\begin{proof}
    By simple algebra we have \begin{align*}
        &\nabla l(\theta) = \frac{1}{n}\sum_{i=1}^n \bigg\{ \frac{\exp(a_i^\top \theta) \cdot ( a_i - h_i) + \exp(b_i^\top \theta)\cdot (b_i - h_i)}{\exp(a_i^\top \theta) + \exp(b_i^\top \theta)}\bigg\} ,\\
        & \nabla^2 l(\theta) = \frac{1}{n}\sum_{i=1}^n \bigg\{\frac{\exp((a_i+b_i)^\top \theta)}{(\exp(a_i^\top \theta)+ \exp(b_i^\top \theta))^2}\cdot (a_i - b_i)(a_i - b_i)^\top\bigg\},
    \end{align*}
    holds for all $\theta\in \RR^d$. By Hoeffding's inequality, we have  $$\PP\big(\max_{i\in[n]}\big\{|a_i^\top \theta^*|, |b_i^\top \theta^*|\big\} \leq \log(2n / \delta) \big) \geq 1-\delta.
    $$
    In the following proof, we will condition on this event. We have \begin{align*}
    \nabla^2 l(\theta^*) &= \frac{1}{n} \sum_{i=1}^n\bigg(\frac{1}{1+ \exp((a_i - b_i)^\top \theta^*)}\cdot\frac{1}{1+ \exp(( b_i - a_i)^\top \theta^*)} \bigg)\cdot (a_i - b_i)(a_i-b_i)^\top\\
    &\succeq \frac{1}{n} \cdot \frac{1}{(1+\exp(\sqrt{\log 2n/\delta}))^2} \sum_{i=1}^n (a_i - b_i)(a_i - b_i)^\top.
    \end{align*}
    In the following we adapt the notation of $\Sigma_x  = \frac{1}{n} \sum_{i=1}^n (a_i - b_i)(a_i - b_i)^\top$, then $\nabla^2 l(\theta^*) \succeq 1/\kappa\cdot \Sigma_x$. To bound $\EE_{x\sim P_a}(|\hat{f}(x) - f^*(x)|)$, we have the following inequality: \begin{align*}
        \EE_{x\sim P_a}[|\hat{f}(x) - f^*(x)|] &= \EE_{x\sim P_a}[|x^\top(\hat{\theta} - \theta^*)|]\\
        &= \EE_{z\sim( A^\top)_\sharp P_a}[|z^\top (A^\top \widehat{ \theta} - \beta)|]\\
        &\leq \underbrace{\EE_{ z\sim( A^\top)_\sharp P_a} [\|z\|_{(\Sigma_z + \lambda I_d)^{-1}}]}_{\operatorname{(i)}} \cdot \underbrace{\|\Delta_z\|_{(\Sigma_z + \lambda I_d)^{-1}}}_{\operatorname{(ii)}}
    \end{align*}
    Here $\Delta_z = A^\top \widehat{\theta} - \beta$. We also denote $\Delta_x = \widehat{\theta} - \theta^*$. To bound (i) note that by Jensen's inequality, we have $$
    \EE_{ z\sim( A^\top)_\sharp P_a} [\|z\|_{(\Sigma_z + \lambda I_d)^{-1}}] \leq \sqrt{\EE_{ z\sim( A^\top)_\sharp P_a}\big[\|z\|^2_{(\Sigma_z + \lambda I_d)^{-1}}\big]} = \sqrt{\operatorname{Tr}\big(\EE_{z\sim( A^\top)_\sharp P_a}[zz^\top]\big) (\Sigma_z + \lambda I_d)^{-1}}.
    $$
    Next we bound (ii). It is easy to prove that $$
    l(\widehat{\theta}) - l(\theta^*) - \nabla l(\theta^*)^\top (\widehat{\theta} - \theta^*) \geq \frac{1}{2\kappa}\|\Delta_x\|_{\Sigma_x}^2.
    $$
By definition of MLE, we have $l(\widehat{\theta}) - l(\theta) \leq 0$. Therefore \begin{align}\label{eq:weight-convex}
    \frac{1}{2\kappa} \|\Delta_x\|_{\Sigma_x}^2 &\leq |\nabla l(\theta^*)^\top (\widehat{\theta} - \theta^*)|\nonumber\\
    & \leq |\nabla l(\theta^*)^\top (A A^\top \widehat{\theta} - \theta^*)| + |\nabla l(\theta^*)^\top(I - A A^\top) (\widehat{\theta} - \theta^*)|.
\end{align}
Recall that $$\nabla l(\theta^*) =  \frac{1}{n}\sum_{i=1}^n  \frac{\exp(a_i^\top \theta) \cdot ( a_i - h_i) + \exp(b_i^\top \theta)\cdot (b_i - h_i)}{\exp(a_i^\top \theta) + \exp(b_i^\top \theta)}, $$ 
since $a_i, b_i $ are in the image set of $A$,  there exists $\alpha\in \RR^d$ such that $\nabla l(\theta^*) = A\alpha$, and we have $$
\nabla l(\theta^*)^\top (I - AA^\top) = \alpha^\top A^\top (I - AA^\top) = 0.
$$
Therefore we have \begin{align}\label{eq:tech-1}
    \frac{1}{2\kappa} \|\Delta_x\|_{\Sigma_x}^2 &\leq |\nabla l(\theta^*)^\top (AA^\top \widehat{\theta} - \theta^* )|\nonumber\\
    & = |(A^\top \nabla l(\theta^*) )^\top \Delta_z |\nonumber\\
    &\leq \|A^\top \nabla l(\theta^*)\|_{(\Sigma_z + \lambda I_d)^{-1}}\cdot \|\Delta_z\|_{\Sigma_z + \lambda I_d}
\end{align}
By $A A^\top (a_i - b_i) = (a_i - b_i) $,  we have \begin{align*}
\|\Delta_x\|_{\Sigma_x}^2 = \Delta_x^\top A \Sigma_z A^\top \Delta_x = \Delta_z^\top \Sigma_z \Delta_z = \|\Delta_z\|_{\Sigma_z}^2,\end{align*}
plug this in \eqref{eq:tech-1}, we have 
\begin{align*}
    \frac{1}{2\kappa} \|\Delta_z\|_{\Sigma_z+\lambda I_d}^2 & \leq \frac{1}{2\kappa} (\|\Delta_z\|_{\Sigma_z}^2 + \lambda \|\Delta_z\|_2^2)\\
    &\leq \|A^\top \nabla l(\theta^*)\|_{(\Sigma_z + \lambda I_d)^{-1}}\cdot\|\Delta_z\|_{\Sigma_z+ \lambda I_d} + \frac{\lambda}{2\kappa} \|\Delta_z\|_2^2 ,
\end{align*}
By  $\|\widehat{\theta}\|_2\leq 1$, we have $ \|\Delta_z\|_2 = \|A^\top \widehat{\theta} - \beta\|_2 = \|\widehat{\theta} - \theta^*\|_2 \leq 2$, and therefore
\begin{align}\label{eq:tech-2}
\|\Delta_z\|_{\Sigma_z+\lambda I_d}^2 \leq 2\kappa \cdot \|A^\top \nabla l(\theta^*)\|_{(\Sigma_z + \lambda I_d)^{-1}}\cdot\|\Delta_z\|_{\Sigma_z+ \lambda I_d}+ {2\lambda}.
\end{align}
To derive an upper bound for $\|\Delta_z\|_{\Sigma_z + \lambda I_d}$, we need to upper bound $\|A^\top \nabla l(\theta^*)\|_{(\Sigma_z + \lambda I_d)^{-1}}$. By Bernstein’s inequality for sub-Gaussian random variables in quadratic form (e.g. see Theorem 2.1 in \cite{hsu2011tail}), we have $$\|A^\top \nabla l(\theta^*)\|_{(\Sigma_z + \lambda I_d)^{-1}} \leq c\cdot\sqrt{\frac{d+\log1/\delta}{n}}$$ for some constant $c$ with probability at least $1-\delta$.
Then we have $$
\|\Delta_z\|_{\Sigma_z+\lambda I_d}^2 \leq 2c\cdot\kappa \cdot \sqrt{\frac{d+\log1/\delta}{n}}\cdot\|\Delta_z\|_{\Sigma_z+ \lambda I_d}+ {2\lambda},
$$
solving which gives $$
\operatorname{(ii)} \leq O\bigg(\sqrt{\kappa^2\cdot \frac{d+\log1/\delta}{n}+ \lambda}\bigg).
$$
Combining (i) and (ii), we prove that $$
\EE_{x\sim P_a} [|\widehat{f}(x) - f^*(x)|] \leq O\bigg(\sqrt{\kappa^2\cdot \frac{d+\log1/\delta}{n}+ \lambda} \cdot \sqrt{ \operatorname{Tr}(\EE_{P_a}[z z^\top] (\Sigma_z + \lambda I_d)^{-1} )}\bigg).
$$
Finally, our result is proved by Lemma \ref{lmm:XtoZ}.
\end{proof}

==> sections/tem_proofs_non.tex <==
\section{Moving from maintext_nonparametric}
\paragraph{Score Matching Error in $s_{\hat w}$} 
\begin{align*}
\frac{1}{T - t_0} \int_{t_0}^T \EE_{x, \hat f} \norm{\nabla_x \log p_t(x, \hat f) - s_{\hat w}(x, \hat f, t)}_2^2 \diff t \leq \epsilon^2_{diff} (N_d).
\end{align*}
Suppose $\nabla_x \log p_t(x, \hat f)$ is within a parametric family $\cS$ and the $s_{w^*} (x, \hat f, t) = \nabla_x \log p_t(x, \hat f)$, then
\begin{equation*}
    \epsilon_{diff} (N_d) = \frac{|\cS|}{\sqrt{N_d}}.
\end{equation*}

\begin{comment}
The score function can be computed as
\begin{align*}
\nabla \log p_t(\xb) = \underbrace{- A \Sigma_t^{-1} A^\top \xb}_{\sbb_\parallel}\underbrace{  - \frac{1}{h(t)} (I_D - AA^\top)\xb}_{\sbb_{\perp}},
\end{align*}
where $\Sigma_t = \diag(\dots,  \alpha^2(t) \lambda_k^2 + h(t) , \dots)$.

One can verify that $\sbb_{\parallel}$ now is linear in $\xb$, whereas $\sbb_{\perp}$ blows up when $t$ approaches $0$. Moreover, only the on-support score $\sbb_{\parallel}$ carries the covariance information of the latent distribution and will guide the distribution recovery.

A closer evaluation further reveals $\pscore$ is Lipschitz continuous, i.e.,
\begin{align*}
\norm{\pscore(\zb_1, t) - \pscore(\zb_2, t)}_{2} \leq \max\{\lambda_d^{-2}, 1 \}\norm{\zb_1 - \zb_2}_2
\end{align*}
for any $t \in [0, T]$ and $\zb_1, \zb_2$, and
\begin{align*}
\norm{\pscore(\zb, t_1) - \pscore(\zb, t_2)}_{2} \leq \max\{\lambda_d^{-2}, 1\} \norm{\zb}_2 |t_1 - t_2|.
\end{align*}
for any $\zb$ and $t_1, t_2 \in [0, T]$. Such properties are essential to develop score approximation and estimation results.
\end{comment}

\paragraph{Regression Error in $\hat f$}
Regression on $\cD_{label}$ leads to 
\begin{align}
\label{equ:rgs_error}
\EE \left[\norm{f^{\star} - \hat{f}}_{L^2(P_{x})}^2\right] \leq \epsilon_{reg} ^2 (N_{r}).
\end{align}

\paragraph{Distribution Shift}
Divergence $\chi^2_{\cG} (p,q)$ is defined as
\begin{align*}
\chi^2_{\cG} (p,q) = \sup_{g \in \cG} \frac{\EE_{p}[g]}{\EE_{q}[g]}.
\end{align*}

\begin{lemma}
\label{lmm:imprv_per_step}
Generating $x$ from $\hat{P}(x | \hat f(x) = a)$ with inputs $a \sim q$ has a guarantee of $f^{\star}(x)$ that
\begin{align}
    \nonumber \EE_{a \sim q} \EE_{x \sim \hat{P}(x | \hat f(x) = a)} [f^{\star}(x)] \geq &\EE_{a \sim q} [a] - 
    2 \norm{\hat f}_\infty \cdot \sqrt{\chi^2_{\cR_{\cS}} (P_{x \hat f}, P_{x|\hat f} \times q)} \cdot \epsilon_{diff} (N_{d})\\
    \label{equ:improvement}&- \sqrt{\chi^2_{\cR_{\cF}} (\hat{p}_q,p)}  \cdot \epsilon_{reg}(N_r).
\end{align}
where $p(x)$ is the density of the marginal distribution of $x$ in $\cD_{label}$, $\hat p_q (x):= \int q(a)\hat{p}(x | \hat f = a)\diff a$ denotes the generated density with input $a \sim q$. We shall take 
\begin{align*}
    \cR_{\cS}&:= \left\{\norm{\nabla_x \log p_t(x, \hat f) - s_w(x, \hat f, t)}_2^2 : s_w \in \cS \right\},\\
    \cR_{\cF}&:= \{|f^* - f|^2: f \in \cF\},
\end{align*}
$\cF$ is the function class to approximate $f^*$.
\end{lemma}

We consider an i.i.d. logged data set consisting of $n$ pairs $(x_i, y_i)$ for $i = 1, \dots, n$. Here $x \in \RR^d$ is the feature, and $y \in \RR$ is a noisy response generated by $y = f^{\star}(x) + \xi$, where $f^{\star}$ is some Lipschitz function and independent noise $\xi$ is Gaussian distributed as ${\sf N}(0, \sigma^2 I)$. We denote the joint sampling distribution on $(x, y)$ as $P_{xy}$. Also we use notation $P_t$ to denote the the joint distribution of $(x,y)$ at time $t$ where $x$ is diffused with Gaussian noise. $p_t(x,y)$ is the corresponding density.
\begin{assumption}
We assume $P_{xy}$ has a density function $p_{xy}$, such that there exists constants $B, C_1, C_2$ verifying $p_{xy}(x, y) \leq (2\pi)^{-(d+1)/2} C_1 \exp\left(-C_2 \norm{x}_2^2 / 2\right)$ whenever $\norm{x}_2 > B$.
\end{assumption}

\begin{assumption}
The score function $\nabla_x \log p_t(x, y)$ of $P_{xy}$ is Lipschitz for any $t \in [t_0, T]$, i.e., there exists a constant $L$, such that for any $x, y$ and $x^{\prime}, y^{\prime}$, it holds
\begin{align*}
\norm{\nabla_x \log p_t(x, y) - \nabla_x \log p_t(x^{\prime}, y^{\prime})}_2 \leq L \norm{x - x^{\prime}}_2 + L\norm{y - y^{\prime}}_2.
\end{align*}
\end{assumption}

\paragraph{Score matching} 
\begin{comment}
We diffuse on $x$ and $y$ jointly. A conceptual loss for score matching is
\begin{align*}
\min_{\theta} \int_{0}^T \EE_{x, y} \left[\norm{\nabla_x \log p_t(x, y) - s_\theta(x, y, t)}_2^2\right] \diff t.
\end{align*}
Note that we have the identity $\nabla_x \log p_t(x | y) = \nabla_x \log p_t(x, y)$. Therefore, the objective function above can also be viewed as estimating the conditional score. To allow practical implementation, we resort to the following equivalent objective,
\begin{align*}
\min_{\theta} \int_{0}^T \EE_{x, y} \left[\EE_{x^{\prime} \sim {\sf N}(\alpha(t)x, h(t)I)}\left[\norm{\nabla_x \log \phi_t(x^{\prime} | x) - s_\theta(x^{\prime}, y, t)}_2^2\right]\right] \diff t,
\end{align*}
whose equivalence is established in Lemma \ref{lemma:obj_equal}.
The remaining analysis follows \url{https://arxiv.org/abs/2302.07194}, with $A = I$.
\end{comment}
We diffuse on $x$ and maintain $y$.  It applies no matter $y$ is a deterministic function of $x$ (i.e. the case where $y = \hat f(x)$) or $y$ is a noisy reward feedback of $f^{\star}(x)$ (i.e. $y = f^{\star}(x) + \xi$) that for $\forall t \not = 0$
\begin{equation}
\label{equ:cdt_score}
    \nabla_x \log p_t(x \mid y) = \nabla_x \log p_t(x , y).
\end{equation}
And all densities in (\ref{equ:cdt_score}) are well-defined. Thus, a conceptual loss of score matching for sampling conditionally is
\begin{align*}
\min_{\theta} \int_{t_0}^T \EE_{x, y} \left[\norm{\nabla_x \log p_t(x, y) - s_\theta(x, y, t)}_2^2\right] \diff t.
\end{align*}

The remaining analysis follows \url{https://arxiv.org/abs/2302.07194}, with $A = I$.

We configure the ReLU network $s_\theta(x, y, t): R^{d+2} \to R^{d}$ by hyperparameters. Specifically, $s_\theta(x, y, t) \in \mathcal{S}_{\mathrm{NN}}\left(L, M, J, K, \kappa, \gamma, \gamma_t\right)$ with
$$
\begin{aligned}
\mathcal{S}_{\mathrm{NN}}\left(L, M, J, K, \kappa, \gamma, \gamma_t\right)=\{ & s_{\theta}(\mathbf{z}, t)=W_L \sigma\left(\ldots \sigma\left(W_1\left[\mathbf{z}^{\top}, t\right]^{\top}+\mathbf{b}_1\right) \ldots\right)+\mathbf{b}_L: \\
& \mathbf{z} = (x,y) \in R^{d+1}, \\
& \text { network width bounded by } M, \sup _{\mathbf{z}, t}\|s_{\theta}(\mathbf{z}, t)\|_2 \leq K, \\
& \max \left\{\left\|\mathbf{b}_i\right\|_{\infty},\left\|W_i\right\|_{\infty}\right\} \leq \kappa \text { for } i=1, \ldots, L, \\
& \sum_{i=1}^L\left(\left\|W_i\right\|_0+\left\|\mathbf{b}_i\right\|_0\right) \leq J, \\
& \left\|s_{\theta}\left(\mathbf{z}_1, t\right)-s_{\theta}\left(\mathbf{z}_2, t\right)\right\|_2 \leq \gamma\left\|\mathbf{z}_1-\mathbf{z}_2\right\|_2 \text { for any } t \in[0, T], \\
& \left.\left\|s_{\theta}\left(\mathbf{z}, t_1\right)-s_{\theta}\left(\mathbf{z}, t_2\right)\right\|_2 \leq \gamma_t\left|t_1-t_2\right| \text { for any } \mathbf{z}\right\},
\end{aligned}
$$
where the network width refers to the maximum dimensions of the weight matrices, $\sigma$ is the ReLU activation, and $\|\cdot\|_{\infty}$ and $\|\cdot\|_0$ denote the maximum magnitude of entries and the number of nonzero entries, respectively. In the sequel, we write $\mathcal{S}_{\mathrm{NN}}\left(L, M, J, K, \kappa, \gamma, \gamma_t\right)$ to reflect the configuration of $\mathrm{f}_\theta$.

\begin{theorem}
\label{thm:NN}
Given an approximation error $\epsilon>0$, we choose $\mathcal{S}_{\mathrm{NN}}$ with
$$
\begin{aligned}
L & =\mathcal{O}\left(\log \frac{1}{\epsilon}+d\right), K=\mathcal{O}\left(2 d^2 \log \left(\frac{d}{t_0 \epsilon}\right)\right) \\
M & =\mathcal{O}\left((1+\beta)^d T \tau d^{d / 2+1} \epsilon^{-(d+1)} \log ^{d / 2}\left(\frac{d}{t_0 \epsilon}\right)\right) \\
J & =\mathcal{O}\left((1+\beta)^d T \tau d^{d / 2+1} \epsilon^{-(d+1)} \log ^{d / 2}\left(\frac{d}{t_0 \epsilon}\right)\left(\log \frac{1}{\epsilon}+d\right)\right) \\
\kappa & =\mathcal{O}\left(\max \left\{2(1+\beta) \sqrt{d \log \left(\frac{d}{t_0 \epsilon}\right)}, T \tau\right\}\right) \\
\gamma & =10 d(1+\beta), \gamma_t=10 \tau
\end{aligned}
$$
where $\tau=\sup _{t \in\left[t_0, T\right]} \sup _{\|\mathbf{z}\|_{\infty}} \leq \sqrt{d \log \frac{d}{t_0 \epsilon}}\left\|\frac{\partial}{\partial t}\left[h(t) \mathbf{s}_{\|}(\mathbf{z}, t)\right]\right\|_2$. Then for any data distribution $P_{x,y}$ satisfying Assumptions \ref{asmp:tail} and \ref{asmp:lipschitz}, there exists an $\overline{\mathbf{s}}_{\boldsymbol{\theta}} \in \mathcal{S}_{\mathrm{NN}}$ such that for any $t \in\left[t_0, T\right]$, we have
$$
\left\|\overline{\mathbf{s}}_{\boldsymbol{\theta}}(x,y, t)-\nabla \log p_t(x,y)\right\|_{L^2\left(P_t\right)} \leq \frac{\sqrt{d}+1}{h(t)} \epsilon .
$$
\end{theorem}

\begin{theorem}
Suppose Assumptions \ref{asmp:tail} and \ref{asmp:lipschitz} hold. We choose $\mathcal{S}_{\mathrm{NN}}$ as in Theorem \ref{thm:NN} with $\epsilon=n^{-\frac{1-\delta(n)}{d+5}}$ for $\delta(n)=\frac{d \log \log n}{\log n}$. Then with probability $1-\frac{1}{n}$, it holds
$$
\frac{1}{T-t_0} \int_{t_0}^T\left\|\widehat{\mathbf{s}}_{ \boldsymbol{\theta}}(x,y, t)-\nabla \log p_t(x,y)\right\|_{L^2\left(P_t\right)}^2 \mathrm{~d} t=\widetilde{\mathcal{O}}\left(\frac{1}{t_0}\left(n^{-\frac{2-2 \delta(n)}{d+5}}+D n^{-\frac{d+3}{d+5}}\right) \log ^3 n\right)
$$
where $\widetilde{\mathcal{O}}$ hides factors depending on $\beta, \log D, d, \log t_0$ and $\tau$ defined in Theorem \ref{thm:NN} .
\end{theorem}

\paragraph{Distribution shift}
Analysis above yields
\begin{align*}
\frac{1}{T - t_0} \int_{t_0}^T \EE_{x, y} \norm{\nabla_x \log p_t(x, y) - s_\theta(x, y, t)}_2^2 \diff t \leq \epsilon_{diff} (N)
\end{align*}
for some $\epsilon$ dependent on sample size $N$ and other hyperparameters.

We translate it to an upper bound under the conditional distribution $P(x | y) \times q_y$, for $q_y$ being a prior distribution on $y$. In particular, we have
\begin{align*}
& \int_{t_0}^T \EE_{y \sim q_y} \EE_{x | y} \norm{\nabla_x \log p_t(x, y) - s_\theta(x, y, t)}_2^2 \diff t \\ & \quad \leq \chi^2_{\cG}(P_{xy}, P_{x | y} \times q_y) \int_{t_0}^T \EE_{x, y} \norm{\nabla_x \log p_t(x, y) - s_\theta(x, y, t)}_2^2 \diff t,
\end{align*}
where divergence $\chi^2_{\cF}$ is defined as
\begin{align*}
\chi^2_{\cF} (P_{xy}, P_{x|y} \times q_y) = \sup_{g \in \cG} \frac{\EE_{P_{xy}}[g]}{\EE_{P_{x|y} \times q_y}[g]}.
\end{align*}
We shall take $\cG$ as $\left\{\norm{\nabla_x \log p_t(x, y) - s_\theta(x, y, t)}_2^2 : s_\theta \in \cS \right\}$.

